Learning Multi-Arm Manipulation Through Collaborative Teleoperation

Imitation Learning (IL) is a powerful paradigm to teach robots to perform manipulation tasks by allowing them to learn from human demonstrations collected via teleoperation, but has mostly been limited to single-arm manipulation. However, many real-world tasks require multiple arms, such as lifting a heavy object or assembling a desk. Unfortunately, applying IL to multi-arm manipulation tasks has been challenging -- asking a human to control more than one robotic arm can impose significant cognitive burden and is often only possible for a maximum of two robot arms. To address these challenges, we present Multi-Arm RoboTurk (MART), a multi-user data collection platform that allows multiple remote users to simultaneously teleoperate a set of robotic arms and collect demonstrations for multi-arm tasks. Using MART, we collected demonstrations for five novel two and three-arm tasks from several geographically separated users. From our data we arrived at a critical insight: most multi-arm tasks do not require global coordination throughout its full duration, but only during specific moments. We show that learning from such data consequently presents challenges for centralized agents that directly attempt to model all robot actions simultaneously, and perform a comprehensive study of different policy architectures with varying levels of centralization on our tasks. Finally, we propose and evaluate a base-residual policy framework that allows trained policies to better adapt to the mixed coordination setting common in multi-arm manipulation, and show that a centralized policy augmented with a decentralized residual model outperforms all other models on our set of benchmark tasks. Additional results and videos at https://roboturk.stanford.edu/multiarm .

==> 1-intro-v2.tex <==
\section{Introduction}
\label{sec:intro}

% Suggested outline (work-in-progress)

% Learning-based manipulation has been promising for single-arm tasks, but multi-arm tasks are more difficult for a number of reasons.

% RL has seen limited success, and often needs to make large assumptions in this setting due to the burden of exploration. 

% Demonstrations can alleviate burden of exploration in these large action spaces - but thus far, demonstration collection in this setting has been infeasible. 

% and having multiple humans collecting this data was something we needed to do in order to enable such data collection - technical innovation - needed to collect demos since these tasks require both arms to act simultaneously


% Learning from human demonstrations collected on multi-arm collaborative tasks poses many interesting questions for imitation learning, especially in mixed-coordination settings (collaboration not required all the time, and since there is a combinatorial blow up of robot states visited, training jointly can overfit to demonstrations seen when robot arms happen to be doing things that are uncorrelated). 

% We use our system to collect data across a range of multi-arm manipulation tasks that require varying degrees of coordination to complete successfully in order to study the effect of inductive biases that impose shared or independent decision making to produce actions for each robot arm.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%IL is awesome. but there is not much demos of multi-arm (multiagent even) collaborative tasks. why? because the system is hard. we present MART

% When collecting data, we observed that, although Collaboration between arms (2 or more) is necessary in many tasks. those tasks do not require them to coordinate all the time

% Our insight: if you don't need to coordinate, why would you try to learn centralized? trying to do it for multiple arms at the same time (when the tasks are mostly single arm most of the time) is just adding complexity (more complexity -> overfitting -> poor performance on unseen task instances due to limited data)

% We propose to try different combinations of centralized|distributed, including variants with hierarchy that can handle better coordination, and a new variant with residuals, that just adds a small modification to coordinate distributed agents

Imitation Learning (IL)~\cite{pomerleau1989alvinn} is a promising paradigm for learning complex robotic manipulation skills by reproducing behaviors from a set of human demonstrations. However, IL has mostly been limited to single-arm manipulation tasks~\cite{zhang2017deep, mandlekar2020learning}. By contrast, many real-world manipulation tasks require multiple robot arms to coordinate to achieve a goal - such as lifting a heavy object, passing an object from one arm to the other, or assembling a desk. 

Multi-arm domains have been relatively unexplored in the context of IL due to the difficulty of collecting human demonstrations. Prior attempts to collect human demonstrations in this setting has suffered from 3 key limitations. Human demonstrations are often collected via teleoperation~\cite{zhang2017deep, mandlekar2018roboturk} by allowing a human to control one or more robotic arms and guide them through a manipulation task, but asking a human to control more than one robotic arm simultaneously can (1) impose significant cognitive burden and (2) is often only possible for 2 robotic arms. Furthermore, (3) such systems can require sophisticated human-control interfaces such as Virtual Reality devices [cite tellex, other bimanual teleoperation we've seen], which are not widely available, consequently limiting the set of users that can participate in data collection.

\begin{figure}
    \centering
    \begin{subfigure}{0.45\textwidth}
      \centering
    \includegraphics[width=\columnwidth]{example-image-a}
    \caption{} 
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
      \centering
    \includegraphics[width=\columnwidth]{example-image-b}
    \caption{} 
    \end{subfigure}
    \hfill
    \caption{a) bbbbbbb, b) dsssllelt. llslslslsls}
    \label{fig:pullfig}
\end{figure}

To address these limitations we present \sysFull (\sysName) - a multi-user data collection platform that allows multiple remote users to simultaneously teleoperate a set of robotic arms and collect demonstrations for collaborative multi-arm tasks. \sysName addresses the limitations of prior multi-arm systems because it (1) frees users from cognitive burden by only having each control a single arm, (2) allows for collecting demonstrations on tasks requiring more than 2 arms, and (3) only requires users to have access to a smartphone and web browser to participate in data collection.

% TODO: do we have to mention RL somewhere in intro? I'd argue we can defer this to related work.
% Due to this difficulty, most work has been limited to autonomous interactive learning techniques such as Reinforcement Learning (RL), which faces the difficult burden of exploration in high-dimensional action spaces, and often requires assumptions on robot capabilities to reduce the search space. 

While \sysName allows for collecting demonstrations from collaborating users on multi-arm manipulation tasks, learning from these demonstrations presents unique challenges for offline imitation learning.
What are the challenges? list here? I don't see them


Different tasks may require varying degrees of coordination between each arm; however, we observed that most behaviors demonstrated by humans using our system consisted of \textit{mixed coordination}, where users would only coordinate their movements at certain task-critical moments.
This is not a challenge, it is an observation


For the other parts of a demonstration, each user would focus on completing their own subtask while ignoring what other users (or robot arms) were doing.


we need to motivate why we are exploring the improvements to standard (Centralized) IL polciies, no? the motivation being system to collect demos --> we observe mixed coordination behavior --> we need to rethink our policy infra to better account for these observations in our collected data




To further investigate this phenomenon, we conducted a user study across several human operators, and observed consistency in . We then proceeded to train standard offline policies 

TODO: we need to make the argument here crisp. What did we observe in our data? How do the methods we investigate, user study we did, experiments we present, tie-in to these observations, the mixed-coordination setting, and our overall goal of learning multi-arm manipulation?

To further investigate this phenomenon, we conduct a user study across several human operators, and analyze how demonstrated behaviors change over time. We also train policies on the collected demonstrations and compare several centralized and de-centralized methods that impose different degrees of coordination when generating robot arm actions. Finally, we present a new algorithm that does X.

TODO: prune the contributions below to 3 (or 4 max) that are related to the TODO above

Concretely, our contributions are as follows:
\begin{enumerate}
    \item We present Multi-Arm RoboTurk (MART), a scalable multi-agent data collection system for gathering human demonstrations on multimanual, collaborative tasks,
    \item We conduct a user study on MART and show that the system is easy to learn and can produce high quality demonstrations after a relatively short operator burn-in period,
    \item We provide a set of realistic multimanual benchmark tasks ranging from the fully decoupled to fully coordinated setting, including a trimanual task that, to our knowledge, is the first of its kind to leverage data from more than two agents,
    \item We evaluate our collected task demonstrations against a variety of baselines and associated variants, and show that a decentralized model formulation aligns better with the underlying data structure and outperforms current centralized IL methods,
    \item We propose and evaluate a novel residual policy framework that leverages the collaborative nature of our collected demonstrations to better synchronize actions between agents and mitigate overfitting, and show that such a method substantially improves base policy performance.
\end{enumerate}


% \begin{itemize}
%     \item Motivate problem of multimanual robot manipulation and learning-based methods for robot manipulation.
%     \item Reinforcement Learning has been applied to bimanual manipulation with some impressive results, but because of high-dimensional action space and large burden of exploration, it has been limited to X (e.g. skills predefined, and search in space of skills).
%     \item However, humans are a natural source of data - that can easily overcome this exploration burden.
%     \item Imitation Learning is great, and has been applied successfully to many domains, and also single-arm robot manipulation. 
%     \item However, there has not been much work on imitation learning for multimanual tasks, because it is difficult to collect data (e.g. interface for controlling multiple arms, cognitive burden on single human). Prior systems have done X for bimanual tasks.
%     \item Our critical insight is to build a data collection system that enables humans to collaboratively solve multimanual tasks, thus easing the cognitive burden of controlling multiple robot arms and generating useful data for learning.
%     \item Due to varying degrees of collaboration in both the tasks, and the data that is collected, this also motivates rethinking the algorithm used to make use of such data.
% \end{itemize}

% Contributions
% \begin{itemize}
%     \item MART: System to collect data
%     \item multi-arm synchronizing residual: Algorithm to leverage data
%     \item Insights of experiments: Experiments (User Study that shows that the system can be used by multiple humans to collect useful data, Algorithm generates impressive results on collected data and outperforms other baselines, and first, to our knowledge, to apply learning-based methods successfully to high-frequency continuous control robot manipulation tasks involving more than 2 arms)
% \end{itemize}

==> table-algo_benchmarks_stripped.tex <==
\begin{table*}
  \caption{\textbf{Results on Experienced Operator Demonstrations}}
  \label{task_benchmark_algo_results}
  \centering
  \begin{tabular}{cccccc}
    \toprule
    Model & \begin{tabular}[c]{@{}c@{}}Two Arm\\ Table Assembly\end{tabular} & \begin{tabular}[c]{@{}c@{}}Two Arm\\ Pick-Place Handover\end{tabular} & \begin{tabular}[c]{@{}c@{}}Three Arm\\ Lifting Wiping\end{tabular} \\
    \midrule
    BC-RNN & $0.0\pm0.0$ & $2.0\pm2.7$ & $56.0\pm6.5$ \\
    HBC & $5.2\pm3.0$ & $16.0\pm3.9$ & $83.7\pm6.5$ \\
    d-HBC & $4.9 \pm 3.1$ & $24.4 \pm 6.4$ & $50.0\pm9.3$ \\
    dh-HBC & $1.3\pm1.6$ & $15.3\pm4.5$ & $62.0\pm8.8$ \\
    dl-HBC & $5.3\pm4.0$ & $10.7\pm4.4$ & $55.3\pm18.2$ \\
    r-HBC (ours) & $\mathbf{10.0\pm2.1}$ & $\mathbf{31.3\pm4.0}$ & $\mathbf{94.0\pm2.5}$ \\
    rd-HBC (ours) & $5.3\pm2.7$ & $26.7\pm4.7$ & $58.6\pm1.6$ \\
    \bottomrule
  \end{tabular}
\vspace{-5pt}
\end{table*}
